The chemical bond as an emergent phenomenon

We first argue that the covalent bond and the various closed-shell interactions can be thought of as symmetry broken versions of one and the same interaction, viz., the multi-center bond. We use specially chosen molecular units to show that the symmetry breaking is controlled by density and electronegativity variation. We show that the bond order changes with bond deformation but in a step-like fashion, regions of near constancy separated by electronic localization transitions. These will often cause displacive transitions as well so that the bond strength, order, and length are established self-consistently. We further argue on the inherent relation of the covalent, closed-shell, and multi-center interactions with ionic and metallic bonding. All of these interactions can be viewed as distinct sectors on a phase diagram with density and electronegativity variation as control variables; the ionic and covalent/secondary sectors are associated with on-site and bond-order charge density wave respectively, the metallic sectorwith an electronic fluid. While displaying a contiguity at low densities, the metallic and ionic interactions represent distinct phases separated by discontinuous transitions at sufficiently high densities. Multi-center interactions emerge as a hybrid of the metallic and ionic bond that results from spatial coexistence of delocalized and localized electrons. In the present description, the issue of the stability of a compound is that of mutual miscibility of electronic fluids with distinct degrees of electron localization, supra-atomic ordering in complex inorganic compounds comes about naturally. The notions of electronic localization advanced hereby suggest a high throughput, automated procedure for screening candidate compounds and structures with regard to stability, without the need for computationally costly geometric optimization.

==> comboSI.tex <==
\title{{\em Supporting Information:} \\ The chemical bond as an
  emergent phenomenon }



\author{Jon C. Golden} \affiliation{Department of Physics, University
  of Houston, Houston, TX 77204-5005}


\author{Vinh Ho} \affiliation{Department of Chemistry, University of
  Houston, Houston, TX 77204-5003} \affiliation{Present address: UT
  Southwestern Medical School; Dallas, TX 75390-9003}

% \author{Joseph Hutchins} \affiliation{Department of Chemistry,
%   University of Houston, Houston, TX 77204-5003}

\author{Vassiliy Lubchenko} \email{vas@uh.edu} \affiliation{Department
  of Chemistry, University of Houston, Houston, TX 77204-5003}
\affiliation{Department of Physics, University of Houston, Houston, TX
  77204-5005} \email{vas@uh.edu}

\date{\today}


% \SectionsOn
% \SectionNumbersOn

% \begin{document}

\maketitle

% \tableofcontents

\setcounter{equation}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{page}{2}
\makeatletter
\renewcommand{\theequation}{S\arabic{equation}}
\renewcommand{\thefigure}{S\arabic{figure}}
\renewcommand{\bibnumfmt}[1]{[S#1]}
\renewcommand{\citenumfont}[1]{S#1}

\section{Potential energy of the
  $\text{AsH}_2-\text{AsH}-\text{AsH}_2$ trimer}

\begin{figure}[h]
  \centering
  \includegraphics[width = 0.9 \figurewidth]{43_As_PES_B.eps}
  \caption{\label{PES} Potential energy surface for the linear 3/4
    trimer AsH$_2$-AsH$_1$-AsH$_2$ as a function the displacement
    $\Delta b \equiv (b_2 - b_1)/2$ of the central As atom off the
    trimer's midpoint and the chain length per bond $b \equiv (b_1 +
    b_2)/2$. The quantities $b_1$ and $b_1$ stand for the As-As bond
    lengths.  The minimum energy contour, shown in bold on the contour
    plot beneath the surface, is determined by minimizing the energy
    at a fixed value of $b$. The surface was obtained using the
    semi-empirical quantum-chemistry package MOPAC with PM6
    parametrization.\cite{JS12}}
\end{figure}

\section{Fluctuation-induced lowering of the symmetry breaking}

The potential energy surface in Fig.~\ref{PES} was obtained using the
Born-Oppenheimer approximation; its minima determine the
zero-temperature location of the nuclei in the classical limit. A
slice of the energy surface in the symmetry-broken region, at a
constant value of the overall trimer length, is exemplified in
Fig.~\ref{fluctuation} by the solid line. Already zero-point vibration
will be sufficient to overcome the barrier separating the two minima
on the bistable energy profile, provided the barrier is sufficiently
low.  To determine qualitatively the trimer length where the barrier
can be still overcome by zero-point vibrations, we consider the
symmetric stretch for concreteness.  A harmonic oscillator with
frequency $\omega$ and mass $m$ exhibits zero-point vibrations of
magnitude~\cite{LLquantum}
\begin{equation} \label{x} x_{T=0} = \left(\frac{\hbar}{m \omega}
  \right)^{1/2}.
\end{equation}
For a quadratic potential whose force constant $\kappa$ matches the
curvature of a symmetry-broken minimum, $\omega = (\kappa/m)^{1/2}$,
where $m$ is the mass of a terminal atom.  Next, we find the value of
the trimer length at which the vibrational magnitude (\ref{x}) exactly
matches the half-width of the barrier separating the two minima, see
the graphical explanation in Fig.~\ref{fluctuation}. This length is
indicated with the asterisk on Fig.~4 of main text.

\begin{figure}[t]
  \centering
  \includegraphics[width =
  \figurewidth]{43_As_trimer_HO_fluctuationB.eps}
  \caption{\label{fluctuation} The solid line is a slice of the
    potential energy function from Fig.~\ref{PES}. The location of the
    slice is chosen so that zero-point vibrations in the harmonic
    potential approximating a metastable minimum on the actual
    potential surface do not exceed, in magnitude, the half-width of
    the barrier separating the two minima on the symmetry broken
    energy surface. }
\end{figure}

\section{Lack of promotion of $3d$ electrons}

It is desirable to check how much the outermost filled $d$ shells are
modified following contraction of the trimer, to test whether
MOPAC's~\cite{JS12} implicit treatment of the core electrons
introduces substantial error.  To this end, we perform an all-electron
HF calculation using the package Orca.~\cite{PN137,Libint2} We
consider a trimer at low density and identify the molecular orbital,
call it X, that primarily consists of the $3d$ atomic orbitals. We
next compress the trimer and, alongside, monitor the contribution of
the atomic $3d$ atomic orbitals to the molecular orbital X. This
contribution is shown in Fig.~\ref{AE_3d} with circles. We observe
that the atomic $3d$ orbitals do not contribute substantially to the
bonding orbitals even at relatively high densities. For the sake of
comparison, we also show the contribution of the atomic $4s$ orbitals
to the very same molecular orbital, with the squares.

\begin{figure}[tph]
  \centering
  \includegraphics[width = 0.7 \figurewidth]{43_As_trimer_Orca_3d_B.eps}
  \caption{Fractional contribution of atomic $3d$ and $4s$ orbitals to
    the trimer's molecular orbital that can identified as primarily
    consisting of $3d$ atomic orbitals at low densities. The
    horizontal axis is the trimer length per bond. The trimer is the
    linear 3/4 molecule AsH$_2$-AsH$_1$-AsH$_2$. The calculations were
    performed with all-electron HF calculation as implemented in the
    package Orca.~\cite{PN137,Libint2} \label{AE_3d}}
\end{figure}

\section{Dependence of symmetry breaking on the $pp\sigma$ bond
  electron count}

The symmetry-breaking graphs for three values of electron count in the
linear trimer AsH$_2$-AsH$_n$-AsH$_2$, $n = 0, 1, 2$, indicate that
the symmetric state becomes less stable when the electron count
differs from its ideal value of four, which yields perfect Lewis
octets for each arsenic. (This situation is realized for a
singly-hydrogenated central arsenic, $n=1$.) In addition, we observe
that in contrast with the situations shown in Fig.~4 and 10 of the
main text, the critical length is no longer the only characteristic
length in the problem. The three bifurcation graphs, shown in
Fig.~\ref{electron_count_reduced}, can still be rescaled so as to
follow one universal curve, inset of
Fig.~\ref{electron_count_reduced}, however doing so requires {\em two}
independent lengths, one needed to fix the lateral position of the
critical point, the other to fix the strength of symmetry breaking.

\begin{figure}[h]
  \centering
  \includegraphics[width = 0.9
  \figurewidth]{AsH2_3atom_electron_count_fork_reducedE.eps}
  \caption{\label{electron_count_reduced} Bond lengths for three arsenic trimers,
    AsH$_2$-AsH$_n$-AsH$_2$ trimer, as functions of the overall trimer
    length per bond. The three cases, $n = 0, 1, 2$, correspond to a
    five, four, and three electron $pp\sigma$ bond bond,
    respectively. Both axes are scaled by the corresponding critical
    bond length $b_c$. Additional scaling is needed to bring the three
    curves to one universal
    dependence. }
\end{figure}

\newpage

\section{Effects of electronegativity variation}

\begin{figure}[h]
  \centering
  \includegraphics[width =
  \figurewidth]{43_interpnictide_trimersD.eps}
  \caption{\label{hetero} Bond lengths for several heteronuclear 3/4
    trimers XH$_2$-YH$_1$-XH$_2$ and YH$_2$-XH$_1$-YH$_2$, as
    functions of the overall trimer length per bond. Both axes are
    rescaled by the corresponding critical radii, no additional
    rescaling of the $\Delta b$ coordinate was performed.}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width =
  \figurewidth]{43_interpnictide_critical_lengthA.eps}
  \caption{\label{rc_hetero} Critical lengths for the heteronuclear
    3/4 trimers XH$_2$-YH$_1$-XH$_2$ and YH$_2$-XH$_1$-YH$_2$ from
    Fig.~\ref{hetero}.   $b_c^>$ and $b_c^<$ correspond to the situation
    where the more electronegative element (X) is placed in the central
    and terminal position, respectively. $b_c^1$ and $b_c^1$ denote
    the critical lengths for the homonuclear trimer
    XH$_2$-XH$_1$-XH$_2$ or YH$_2$-YH$_1$-YH$_2$.}
\end{figure}

%Several molecular examples are considered in
%Figure~\ref{epsilon_variation} representing a range electronegativity
%difference between the central and terminal atoms spanning zero to
%nearly 2 ev. To offset the effects of atomic number and ion size on
%the actual transition location, we have normalized the difference
%between the spatial and electronic critical lengths by the spatial
%critical length $b_c^{\mathrm{(spatial)}}$ pertinent to each molecule.
%\begin{figure}[h]
%  \centering
%  \includegraphics[width =
%  \figurewidth]{43_Trimer_electronegativity_variation_A.eps}
%  \caption{Dimensionless separation length $\delta$ between the
%    electronic and spatial transitions, normalized by the critical
%    bond length $b_c^{\mathrm{(spatial)}}$ to suppress to the atomic
%    number and size influences, shown as a function of
%    electronegativity variation $\varepsilon$ between the terminal and
%    central atoms.\label{epsilon_variation}}
%\end{figure}

\newpage

\section{Example of the Landau-Ginzburg free energy near a 1st order
  transition}

\begin{figure}[h]
  \centering
  \includegraphics[width =
  \figurewidth]{TeSbTe_A.eps}
  \caption{Slices of the full energy surface at $b=\text{const}$, for
    three values of the latter, for the 3/4 heterotrimer TeH-Sb-TeH
    near the symmetry breaking transition. The three distinct minima
    are present in one slice but are very shallow; the corresponding
    barriers would be easily erased by already zero-point vibrations.}
\end{figure}

\section{Re-parametrization of antimony in MOPAC}

MOPAC evaluates the matrix elements of the Hamiltonian using a
approximation, in which their coordinate dependence is fully
determined by coordinate dependence of the overlaps of the
corresponding (atomic) basis orbitals.~\cite{WolfsbergHelmholz}
Figs.~\ref{shrinking1}-\ref{shrinking4} show the wavefunction overlaps
involving the pseudo-antimony with itself and with arsenic, and, for
comparison, with MOPAC's built-in As-As overlaps. MOPAC uses
Slater-type orbitals. The lengthscale $\xi$ refers to the orbital
exponent that determines the inverse rate of the exponential decay of
the wavefunction overlap.

\begin{figure}[h]
  \centering
  \includegraphics[width = 0.7 \figurewidth]{As_Sb_ss_overlap.eps}
  \caption{\label{shrinking1} The $s$ wavefunction overlaps as 
    functions of separation for As-As, As-Sb and Sb-Sb bonds.}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width = 0.7 \figurewidth]{As_Sb_sp_overlap.eps}
  \caption{\label{shrinking2} The $sp$ wavefunction overlaps as
    functions of separation for As-As and As-Sb bonds.}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width = 0.7 \figurewidth]{As_Sb_pp_overlap.eps}
  \caption{\label{shrinking3} The $pp$ wavefunction overlaps as 
    functions of separation for As-As and As-Sb bonds.}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width = 0.7 \figurewidth]{As_Sb_dd_overlap.eps}
  \caption{\label{shrinking4} The $dd$ wavefunction overlaps as
    functions of separation for As-As, As-Sb and Sb-Sb bonds.}
\end{figure}

\newpage

\section{Re-parametrization of MOPAC PM6 basis set under pressure}

MOPAC employs one, Slater-type wave function per atomic orbital with a
fixed extent. The latter is optimized to match geometries and
formation enthalpies at normal conditions. Such a single-wavefunction
parametrization may not be quantitative at high pressures, however. To
test for this potential complication, we have solved for the HF
wavefunctions of the 3/4, homonuclear arsenic trimer using a Quantum
Chemistry package that approximates atomic wavefunctions with a linear
combination of five Gaussian type functions (GTF); the widths of the
individual Gaussians span a substantial range. We then monitor the
coefficients at individual GTF's as functions of density.

\begin{figure}[h]
  \centering
  \includegraphics[width = 0.8 \figurewidth]{43_As_trimer_AEf.eps}
  \caption{\label{shrinking} Composition of the $p$ atomic orbital in
    $pp\sigma$ bonding MO in arsenic trimer as a function of
    interatomic separation, from ORCA aug-cc-pvtz all electron HF
    calculations.}
\end{figure}

Fig.~\ref{shrinking} shows the makeup of a $p_{z}$ atomic orbital in
the $pp\sigma$ bond as a function of the As-As bond length. The
vertical axis shows the square of coefficients $c_{1}$-$c_{5}$, 1
representing the least extended and 5 representing the most extended
Gaussian function. As the ion cores approach each other, the
wavefunction becomes less diffuse; $c_{3}$ grows while $c_{5}$
shrinks.

In addition, MOPAC's default parametrization of the hard core
repulsion between the ionic cores may not be fully adequate in the
broad density range of interest. (Within the MOPAC PM6 method, the
Pauli repulsion between closed shells is approximated with Voityuk's
diatomic expression\cite{VR104}.)

\begin{figure}[h]
  \centering
  \includegraphics[width = 0.8
  \figurewidth]{orbital_exponent_scale_fz.eps}
  \caption{Orbital exponent scaling function behavior for simple cubic
    and body centered cubic lattices, illustrated using the ratio of
    the scaled exponent $\xi(a)$ to the default PM6 value
    $\xi_{0}$\label{fz}}

\end{figure}

The above notions are consistent with our findings that MOPAC's
built-in parametrization does not correctly locate the transition
densities for the sc-to-bcc transition in elemental arsenic
(sc='simple cubic', bcc='body-centered cubic'). As a stopgap solution,
we have introduced additional parametrization to both the orbital
exponent $\xi$ of the wavefunction overlap and the parameter $\chi$
which is the overall scaling factor for the core-core repulsion. The
resulting parametrization of $\xi$ and $\chi$ as functions of the
lattice constant $a$ is shown in Figs.~\ref{fz} and \ref{fx},
respectively.  Using the common tangent method, Fig.~\ref{pt}, we
confirm a first order simple cubic to body centered cubic transition
at 97~GPa and the experimental volume fraction $V_T/V_0$ reported in
high pressure xray crystallography studies. The equation of state for
bcc-As can be found in Ref.~\cite{PhysRevB.51.597} Note there is a
coexistence region between the simple cubic and bcc phases where the
structure is thought to be incommensurate.~\cite{PhysRevB.77.024109}
In the absence of information on the pressure dependence of the
density within the inter-transition region, we use a simple linear
form of the scaling functions in that region. By the same token, the
above re-parametrization is consistent with a continuous transition
between rhombohedral and simple cubic at 25 Gpa, while the
experimental $V_T/V_0$ is also recovered.~\cite{PhysRevB.41.5535}

\newpage
 
\begin{figure}[h]
  \centering
  \includegraphics[width = 0.8 \figurewidth]{core-core_scale_fx.eps}
  \caption{Linear core-core repulsion pseudo-potential scaling
    functions for simple cubic and body centered cubic
    lattices.\label{fx}}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width = 0.8
  \figurewidth]{AsSb_PM6_bcc_cubic_PTb.eps}
  \caption{Common tangent construction of the first order simple cubic
    to bcc phase transition for the pseudo-arsenic material at
    $\epsilon$ = 0. The density index shown on the horizontal axis is
    an internal variable used in the PM6 calculations to set a common
    density in both the simple cubic and bcc lattices, the values of
    $18$ and $30$ marked with vertical dashed lines correspond to the
    experimentally observed boundaries of the first order
    transition.\label{pt}}
\end{figure}

\newpage

\section{Hysteretic behavior of the energy as a function of the
  electronegativity variation}

We have found that the self-consistent Hartree Fock procedure does not
always converge to the variational bound on the true ground state that
is actually accessible to MOPAC. Given this uncertainty, we have
performed many $\epsilon$ ``sweeps,'' whereby the electronegativity
differential $2 \epsilon$ is cycled between values of 0 and 8 eV.  The
result of this protocol is exemplified in Fig.~\ref{busy_plot}. The
cycling was terminated when two consecutive sweeps back and forth did
not produce a jump to a lower yet term.

\begin{figure}[h]
  \centering
  \includegraphics[width =
  \figurewidth]{AsSb_cubic_i33_busy_plotA.eps}
  \caption{\label{busy_plot} A sample of the ``sweep'' protocol
    demonstrating an overshoot of a term crossing. Labels ``met'' and
    ``ionic'' correspond with sweeps that begin at the $\epsilon = 0$
    and $\epsilon = 4$~eV ends of the $\epsilon$ range.}
\end{figure}

\newpage

\section{Stability of the simple cubic structure to rhombohedral
  distortion}

Fig.~\ref{cubic_i51_k1} shows the energy of a 64 atom pseudo-arsenic
solid as a function of the magnitude of a distortion toward the
rhombohedral lattice, as in Fig.~12 of the main text. Hereby, we shift
the anionic and cationic sublattice relative to each other along the
[111] direction. At the higher of the two densities shown in
Fig.~\ref{cubic_i51_k1}, the presence of a central minimum indicates
that the distortion is destabilizing. This is approximately the
density where the rhombohedral-to-simple cubic transition is observed
experimentally.~\cite{PhysRevB.41.5535}

\begin{figure}[h]
  \centering
  \includegraphics[width = 0.9
  \figurewidth]{AsSb_cubic_PM6_i51_k1.eps}
  \caption{Onset of susceptibility to small distortion towards
    rhombohedral structure, as probed by relative shift of the
    cationic and anionic sublattices comprising the rock-salt
    structure of the pseudo di-pnictogen
    compound.\label{cubic_i51_k1}}
\end{figure}

\section{Decrease in $sp$-mixing in rhombohedral arsenic with density}

To examine $sp$-mixing in rhombohedral arsenic we have used the
projected crystal orbital Hamilton population (pCOHP) analysis tool
Lobster~\cite{DB97,DTD115,MDTD34} to extract chemical bonding
information from the results of plane-wave calculations.  pCOHP is a
close relative of the crystal orbital overlap population (COOP)
analysis, originally known as overlap population density of states
(OPDOS).

Density functional theory (DFT) calculations were performed in the
generalized gradient approximation (GGA) parameterization of Perdew,
Burke and Emzerhof~\cite{PBE38,CA45} using the Vienna ab-initio
Simulation Package (VASP) version 5.3~\cite{KH47,KF6,KJ59} with
Blochl's projector augmented-wave (PAW) method employed for the core
states.~\cite{PEB50} In the rhombohedral structure at ambient
pressure, there is a gap between the $s$ and $p$ contributions to the
overall density of bonding states, as shown in Fig.~\ref{As_COHP}.

\begin{figure}[h]
  \centering
  \includegraphics[width = \figurewidth]{rhomb_to_cubic_As_COHP.eps}
  \caption{The dashed line indicate a gap between portions of the
    electronic density of states primarily associated with bonding $s$
    and $p$ electrons, in rhombohedral arsenic at normal
    conditions. The red boxes show $s$ and $p$ contributions to the
    density of bonding states.\label{As_COHP}}
\end{figure}

We next compress the unit cell while simultaneously reducing the
rhombohedral distortion until we reach the density where the phase
transition to simple cubic is observed experimentally. The width of
the gap region shown in Fig.\ref{As_COHP} shrinks with density before
vanishing at the transition. We interpret this shrinking as a
decreased mixing between the $s$ and $p$ bonding sub-systems.

\begin{figure}[h]
  \centering
  \includegraphics[width = \figurewidth]{rhomb_to_cubic_As_sp_mixing.eps}
  \caption{The dependence of the $sp$ from Fig.~\ref{As_COHP} as the
    sample is compressed and deformed toward the simple cubic
    structure.\label{sp_mixing_compressed}}
\end{figure}

\newpage

\section{Ab-initio verification of electronic symmetry breaking for
  symmetric AsH$_2$-AsH-AsH$_2$ trimer}

To verify the apparent change in the bond characteristics, as implied
by the MOPAC-based, LMO analysis, we have obtained variational HF
solutions for the symmetric 3/4 trimer AsH$_2$-AsH-AsH$_2$ using the
6-311G basis within Gaussian 09.\cite{g09} The latter Quantum Chemistry
package provides an alternative interpretational tool to analyse
bonding, viz., via the NBO 6.0 Natural Bond Orbital (NBO).~\cite{NBO6}
Natural Bond Orbitals (NBOs) are an orthonormal set of localized
orbitals in the form of core orbitals (CR) bonding orbitals (BD), lone
pairs (LP) and multi-center orbitals (nC).  The first three orbital
types are Lewis-type orbitals. The procedure attempts to maximize the
occupancy of these Lewis orbitals, the remaining electronic density
assigned to non-Lewis, multi-center orbitals. 

\begin{figure}[b]
  \centering
  \includegraphics[width=.9 \figurewidth]{As3H5_320A_NBO6.eps}
  \caption{Fragment of the output of the NBO6 analysis within
    Gaussian09 for spatially-symmetric trimer at
    $b=3.2$~\AA.\label{320A_NBO6}}
\end{figure}

Similarly to the LMO-based conclusions in the main text, we have
detected a qualitative change in the NBOs by which a three-center
orbital and associated lone pair emerge for sufficiently long
trimers. Fragments of the corresponding output files just before and
after the transition are provided in Figs.~\ref{320A_NBO6} and
\ref{330A_NBO6}, respectively. For the reader's convenience, we framed
the results of the final iteration of the NBO procedure, which
indicate that following the transition, the number of two-center bonds
decreased by 2 while a three-center bond and a lone pair appeared. See
also the framed entry in Fig.~\ref{330A_NBO6} for orbital 52. The
configurations in Figs.~\ref{320A_NBO6} and \ref{330A_NBO6} correspond
to the As-As bond lengths $b = 3.2$ and $3.3$~\AA, respectively, which
is less than but reasonably close to MOPAC's figure $b \approx
3.6$~\AA. Importantly, this figure is still much longer than what is
expected for the covalent As-As bond, i.e., 2.4~\AA~or so.

\begin{figure}[h]
  \centering
  \includegraphics[width=\figurewidth]{As3H5_330A_NBO6.eps}
  \caption{Fragment of the output of the NBO6 analysis within
    Gaussian09 for spatially-symmetric trimer at
    $b=3.3$~\AA.\label{330A_NBO6}}
\end{figure}

\newpage

\section{Walsh diagram of the molecular terms of the trimer
  AsH$_2$-AsH-AsH$_2$ as functions of the trimer length}

\begin{figure}[H]
  \centering
  \includegraphics[width = 0.9\figurewidth]{AsH2_3atom_i500_i930_terms_C.eps}
  \caption{MOPAC-derived molecular orbital terms for the
    AsH$_2$-AsH-AsH$_2$ trimer as functions of the As-As bond length
    $b$. The vertical dashed line indicates the bond length at which
    the LMO transition takes place.\label{3/4 MO Walsh}}
\end{figure}

\newpage

\section{Bonding from the viewpoint of localized molecular orbitals}

\label{LMO}

We will characterize bonding using the localized molecular orbital
(LMO) formalism. Originally inspired by symmetry adapted orbitals in
relatively symmetric molecules, the localized molecular orbitals can
be assigned for arbitrary geometries: Given a set of {\em occupied}
molecular orbitals $\psi_i$, one transforms to an alternative set of
orthonormal orbitals $\chi_j$ such that a certain quantity reflecting
the self-repulsion within individual new orbitals is
maximized.\cite{SB32, ER35, VN56, PS78} Specifically, here we adhere
to the Edmiston and Ruedenberg approach~\cite{ER35}, whereby one
maximizes the quantity $D_\chi \equiv \sum_j \int d^3 \br_1 d^3 \br_2
|\chi_j(\br_1)|^2 V(r_{12}) |\chi_j(\br_2)|^2$ or, equivalently,
minimizes the mutual repulsion among distinct orbitals in the form of
the quantity: $\sum_{j<k} \int d^3 \br_1 d^3 \br_2 |\chi_j(\br_1)|^2
V(r_{12}) |\chi_k(\br_2)|^2$. The function $V(r_{12})$ stands for a
purely repulsive potential energy function.  The LMOs are generally
not eigenfunctions of an effective one-particle Hamiltonian, such as
that arising in the Hartree-Fock (HF) approximation. Instead, they
represent an attempt by an interpreter to redistribute (the already
bound) electrons among orthonormal, maximally localized orbitals, each
of which thus binds together the smallest number of atoms. The latter
number serves as a lower bound on the number of centers in a bond; the
bound is not unique because it depends on the specific choice of the
% (The quantity $\sum_{mn} \int d^3 \br_1 d^3 \br_2 |\chi_m(\br_1)|^2
% V(r_{12}) |\chi_n(\br_2)|^2$ is independent of the basis choice, of
% course.)
test function $V(r_{12})$, which is made according to one's
convenience and computational means. For instance, $V(r_{12}) =
r_{12}^{-1}$ implies localization with respect to (non-screened)
Coulomb repulsion. A more computationally convenient choice is
$V(r_{12}) = \delta(\br_{12})$, which simply yields $D_\chi = \sum_j
\int d^3 \br |\chi_j(\br)|^4$.

The above procedure is significantly simplified when the one-electron
energy function is diagonalized while neglecting the overlap between
distinct atomic orbitals, as is the case for certain semi-empirical
approximations.~\cite{PS78} Hereby, one can present the integral $\int
d^3 \br |\chi_j(\br)|^4$ as a sum over distinct atoms: $\sum_A \int_A
d^3 \br |\chi_j(\br)|^4$, where the individual integrations are over
regions occupied by distinct atoms. Each such integration yields a
quantity that scales inversely proportionally with the atom's
volume. Insofar as we are interested in the partitioning of the
electrons between atoms, irrespective of the extent of the atomic
orbitals, the above sum can be profitably replaced by a
(dimensionless) expression, viz.:
\begin{align} \label{partition1} \int d^3 \br |\chi_n(\br)|^4 &=
  \sum_A \int_A d^3 \br |\chi_n(\br)|^4 \to \\ \label{partition2} n_j
  &\equiv \sum_A \left( \sum_{\lambda_A} C^2_{\lambda_A j} \right)^2,
\end{align}
where we have expanded the localized orbital $\chi_j(\br)$ in terms of
the atomic orbitals $\phi_{\lambda_A}$:
\begin{equation} \label{chiExp} \chi_j(\br) = \sum_A \sum_{\lambda_A}
  C_{\lambda_A j} \phi_{\lambda_A}
\end{equation}
and the index $\lambda_A$ labels the atomic orbitals on atom $A$. As
already mentioned, $\int dV \phi_\lambda \phi_\mu = \delta_{\lambda
  \mu}$, implying $\sum_A \sum_{\lambda_A} C^2_{\lambda_A n} = 1$. The
quantity $n_j$ from Eq.~(\ref{partition2}) clearly provides the
participation number of distinct centers to the localized orbital $j$,
and is appropriately called the {\em bond-center number}.~\cite{PS78}
For a lone pair, one automatically gets $n = 1$. For a two-center
bond, the MO and LMO are equal: $\chi = \psi = \alpha \phi_1 + \beta
\phi_2$, ($\alpha^2 + \beta^2 = 1)$; the bond center number, $n =
[\alpha^{-4} + (1 - \alpha^2)^{-2}]^{-1}$, is maximized at 2 for a
covalent bond, $\alpha = 1/\sqrt{2}$, and is minimized at the lone
pair value 1 for a purely ionic bond, $\alpha = 0, 1$. For a linear
trimer with two equivalent bonds and one orbital per center, one may
use the H\"{u}ckel energy function:
\begin{equation}\label{Htrimer}
  \widehat{H} = - \left(  {\begin{array}{*{20}{c}}
        0 & \beta & 0 \\
        \beta & 0 & \beta\\
        0 & \beta &  0 \end{array}} \right).
\end{equation}
The corresponding MO's are shown graphically in Fig.~\ref{H3}(a).  The
lowest-energy MO is $\psi_1 = \phi_1/2 + \phi_2/\sqrt{2} + \phi_3/2$
and the (formally) non-bonding MO is $\psi_2 = (\phi_1 -
\phi_3)/\sqrt{2}$. If only the {\em ground} state MO contributes to
bonding, one gets $n = 8/3$. This value is less than three, in
reflection of the non-uniform distribution of charge among the three
centers, viz., $25\%$, $50\%$, and $25\%$ respectively.  The partially
ionic character of the three-center bond for a linear trimer made of
otherwise equivalent atoms was noted a while ago by
Musher.~\cite{MusherAngew1969} (For comparison, the bond-center number
for a three-center bond with three equivalent centers, $\chi = \psi =
(\phi_1 + \phi_2 + \phi_3)\sqrt{3}$ exactly equals $3$.) In the case
when MO2 is actually bonding, there are two LMOs. Direct computation
shows $\chi_{1, 2} = (\psi_1 \pm \psi_2)/\sqrt{2}$, the two shown
graphically in Fig.~\ref{H3}(b). The two LMOs are equivalent in that
they are mirror images of each other, up to the sign, and each can be
associated with a one-electron energy $(E_1 + E_2)/2$. (Generally, to
the $j$-th LMO $\chi_j = \sum_{l} c_{jl} \psi_l$, one may associate an
energy $E_j = \sum_{l} c_{jl}^2 E_l$, where the summations are over
the occupied MOs.) The bond number for each of the two LMOs is
$n_{1,2}= 32/19$, which is just short of 2. This (modest) deficit is,
again, due to the non-uniform distribution of charge among the three
centers. Still, insofar as the bond-center numbers for the two LMOs
are numerically close to 2, the 3 center/4 electron bond can be
thought of as two adjacent two-center bonds.

\begin{figure}[t]
  \centering
  \includegraphics[width = .95 \figurewidth]{H3_d.eps}
  \caption{\label{H3} {\bf (a)} Graphical representation of the
    eigenvectors of the three-orbital, H\"{u}ckel energy function
    (\ref{Htrimer}). {\bf (b)} The localized molecular orbitals (LMOs)
    corresponding with panel (a). Note the two orbitals have the same
    energy, $(E_1 + E_2)/2$.}
\end{figure}

A useful pattern emerges from the above trimer example already at the
H\"{u}ckel level, as in Fig.~\ref{H3}: If the two-center bonds
comprising the three-center bond are equivalent and the two bonding
molecular orbitals have opposite parity, the two resulting LMOs are
necessarily mirror images of each other. (This pattern does not
necessarily hold when the number of MOs exceeds two, whether that
number is even or odd.) If only one LMO is present, on the other hand,
it must be either odd or even with respect to reflection in the
symmetry plane.

As a measure of the bond order for a two-center bond connecting atoms
A and B, one may evaluate the number of electrons shared by these
atoms according to:~\cite{APS627}
\begin{equation} \label{BOdef} B_{AB} \equiv \sum_{\lambda_A \!, \,
    \lambda_B} P^2_{\lambda_A \lambda_B},
\end{equation}
where $P_{\lambda \mu}$ is the density matrix:
\begin{equation} P_{\lambda \mu} \equiv 2 \sum_i
  \widetilde{C}_{\lambda i} \widetilde{C}_{\mu i},
\end{equation}
the summation being over the occupied MOs, and the $\widetilde{C}$s
are the expansion coefficients for the MOs in terms of the atomic
orbitals:
\begin{equation} \label{psiExp} \psi_i(\br) = \sum_A \sum_{\lambda_A}
  \widetilde{C}_{\lambda_A i} \phi_{\lambda_A}.
\end{equation}
The quantity in Eq.~(\ref{BOdef}) is often called the ``Wiberg bond
index.''\cite{Armstrong73} For a lone pair, $B = 0$ automatically. For
a two-center bond, $\psi = \alpha \phi_1 + \beta \phi_2$, $B_{AB} = 4
\alpha^2 (1-\alpha^2)$; it varies between 0 and 1, the two extremes
corresponding to a purely ionic and covalent bond, respectively. For
the trimer from Eq.~(\ref{Htrimer}), the bond orders are $B_{12} =
B_{12} = 1/2$, and $B_{13} = 1/4$, whether the number of the bonding
MO's is one or two.  We thus conclude that the bond order defined in
Eq.~(\ref{BOdef}) reflects, to some extent, the deviation of the
bonding in Fig.~\ref{H3} from a collection of two-center bonds, since
$1/2+1/2+1/4 = 1.25 > 1$.

To gain additional insight, one may quantify the bonding contribution
of an individual LMO, $j$, by evaluating the expectation value of the
density matrix for the orbital, see ``Localization Theory'' in the
online MOPAC Manual~\cite{MOPACmanual}
\begin{equation} \label{BcontDef} C^\text{(bond)}_{jj} \equiv \la
  \chi_j | \widehat P | \chi_j \ra = 2 \sum_{\lambda \mu} C_{\lambda
    j} C_{\mu j} P_{\lambda \mu},
\end{equation}
where in the sum above, terms pertaining to the same atom are
excluded.  The bonding contribution for a lone pair is automatically
$0$. For a two-center bond $\chi = \psi = \alpha \phi_1 + \beta
\phi_2$, $C^\text{(bond)} = 8 \alpha^2 (1-\alpha^2)$, which is simply
the Wiberg bond index times two. Likewise, the trimer from
Eq.~(\ref{Htrimer}) in the one-LMO arrangement yields $C^\text{(bond)}
= 2.5$. The two-LMO arrangement leads to $C^\text{(bond)}_{11} =
C^\text{(bond)}_{22} = 1.25$, so that the total bond contribution is,
again, $2.5$. Thus based on the bond index and bond contribution
analysis, the bond order for the H\"uckel trimer is not sensitive to
whether MO2 is regarded as bonding or non-bonding. We shall see that
the two analyses give different results in more complicated
situations.

\newpage

\section{The eventual dissociation of the trimer, from the LMO
  perspective}

\begin{figure}[h]
  \centering
  \includegraphics[width = 1.2
  \figurewidth]{AsH2_3atom_i87_i88_MOs_b.eps}
  \caption{The bonding LMOs are shown for the AsH$_2$-AsH-AsH$_2$ for
    two values of the bond length, (a) $b = 3.74$~\AA~ and (b) $b =
    3.76$~\AA.}
\end{figure}

\section{A realization of a 5-center localized molecular orbital}

\begin{figure}[h]
  \centering

  \includegraphics[width = 1.4\figurewidth]{AsH2_11atom_MO_38A.eps}

  \includegraphics[width = 1.4 \figurewidth]{AsH2_11atom_LMO_38A.eps}

  \caption{MOPAC-derived $pp\sigma$ molecular orbital (top) and
    corresponding localized molecular orbital (bottom). All nearest
    neighbor As-As bond lengths are equal to $3.39$~\AA. The hydrogens
    are constrained in the same fashion as for the 3/4 trimer in the
    main text.}
\end{figure}

\newpage

\section{The 20-member ring hosts a charge-density wave (CDW)}

\begin{figure}[h]
  \centering
  \includegraphics[width = 0.9
  \figurewidth]{AsH2_20atom_ring_ground_state_onsite_s.eps}
  \caption{An example of a charge density wave in the 20-member ring
    (AsH$_{2}$)$_{20}$, as inferred from the diagonal entries of the
    density matrix, see main text. The specific bond length,
    $b=2.73$~\AA, corresponds with the ground state configuration of
    the non-dimerized 20 member ring at the ground state configuration
    indicated by the asterisk in Fig.~14 of main text.\label{CDW}}
\end{figure}

\newpage

\section{The 20-member ring becomes unstable toward dimerization for
  bond lengths exceeding 2.5~\AA}

\begin{figure}[h]
  \centering
  \includegraphics[width = 0.9
  \figurewidth]{AsH2_20_atom_ring_i52_dimerization_A.eps}
  \caption{Electronic energy of the 20-member ring (AsH$_{2}$)$_{20}$
    as a function of the dimerization strength. The latter is
    indicated by the length difference between the longer and shorter
    bond. The average bond length is kept steady at
    $2.50$~\AA. \label{stable}}
\end{figure}


\begin{figure}[h]
  \centering
  \includegraphics[width = 0.9
  \figurewidth]{AsH2_20_atom_ring_i55_dimerization_A.eps}
  \caption{Electronic energy of the 20-member ring (AsH$_{2}$)$_{20}$
    as a function of the dimerization strength. The latter is
    indicated by the length difference between the longer and shorter
    bond. The average bond length is kept steady at
    $2.58$~\AA.  \label{bistable}}
\end{figure}

\newpage

\section{Additional examples of localized molecular orbitals near the
  ground state length of the non-dimerized 20-member ring}

\begin{figure}[h]
  \centering \subfigure{\includegraphics[width = 0.45
    \figurewidth]{AsH2_20_atom_ring_dimer_i55_chiral_LMOs.eps}} \hspace{2cm}
  \subfigure{\includegraphics[width = 0.45
  \figurewidth]{AsH2_20_atom_ring_dimer_i61_ground_state_LMOs.eps}}
\caption{{\em Left}: The LMOs near the mechanical stability limit of
  the 20-member ring (AsH$_2$), a higher energy HF solution than the
  one visualized in Fig.~13 of main text, regime III; $b =
  2.58$~\AA. {\em Right}: The LMOs for the ground state configuration
  of the non-dimerized 20 member ring at the ground state
  configuration indicated by the asterisk in Fig.~14 of main text.}
\end{figure}

\newpage

\section{Molecular geometry for the $AsH_{2}-AsH-AsH_{2}$ and $AsH_{2}-AsH_{2}-AsH_{2}$ trimers}

\begin{figure}[h]
  \centering
  \includegraphics[width = 0.7 \figurewidth]{As_trimers_c.eps}
  \caption{\label{As_trimers} The trimers AsH$_2$-AsH-AsH$_2$ (panel
    (a)) and AsH$_2$-AsH$_2$-AsH$_2$ (panel (b)), corresponding to
    3-center/4-electron and 3-center/3-electron $pp\sigma$ bond.}
\end{figure}

\section{Spatial symmetry breaking in the $AsH_{2}-AsH-AsH_{2}$ trimer}

\begin{figure}[h]
  \centering
  \includegraphics[width = \figurewidth]{43_As_trimer_b1b2.eps}
  \caption{\label{b1b2} The equilibrium values of the As-As bond
    lengths for a fixed value of the overall trimer length, according
    to the dashed line on the associated potential energy surface in the main text; {\bf (a)} as functions of
    the trimer length per bond, {\bf (b)} plotted parametrically, for
    the longer bond vs. the shorter bond.}
\end{figure}

\newpage

\section{Term crossing upstream of the LMO transition in the $AsH_{2}-AsH-AsH_{2}$ trimer}

\begin{figure}[h]
  \centering
  \includegraphics[width = 0.8
  \figurewidth]{AsH2_3atom_i500_i930_terms_MO9_MO10_D.eps}
  \caption{\label{MOexplanation} The energies of the MOs responsible
    for the $pp\sigma$ bond and the lone pair on the central arsenic,
    as functions of the As-As bond length $b = b_1 = b_2$, for the 3/4
    case. The vertical dashed line indicates the location of the LMO
    transition in Fig. 13 of the main text.}
\end{figure}

\section{Potential energy of the $AsH_{2}-AsH-AsH_{2}$ trimer}

\begin{figure}[h]
  \centering
  \includegraphics[scale=0.25]{33_As_trimer_ROHF_i1_i100_contour_d.eps}
  \caption{\label{33PES} The contour plot of the potential energy of
    the 3/3 trimer, Fig.~\ref{As_trimers}(a), as a function of the
    trimer length per bond $b \equiv (b_1 + b_2)/2$ and the distance
    of the center arsenic from the midpoint between the terminal
    arsenics, $\Delta \equiv (b_1 - b_2)/2$.  The metastable symmetric
    configuration is marked by the filled red circle. The dashed,
    bifurcating graph shows the minimum energy at fixed value of $b$.}
\end{figure}

\newpage

\section{Localized molecular orbital analysis of the 3 electron
multi-center bond}

\begin{figure}[h]
  \centering
  \includegraphics[width = \figurewidth]{AsH2_trimer_ROHF_BOd.eps}
  \caption{\label{33BO} The bonding contribution of the LMOs as
    functions of the As-As bond length $b = b_1 = b_2$, for the 3/3
    molecule.}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\figurewidth]{33_As_trimer_NBO_Ni_WibergA.eps}
  \caption{\label{33BI} Displayed as functions of the As-As bond
    length $b = b_1 = b_2$: {\bf (a)}, the bond center number for the
    LMOs from Fig.~\ref{33BO}; {\bf (b)}, the Wiber bond index. Note
    the latter is computed using the density matrix and does not rely
    on the localization procedure.}
\end{figure}

\newpage

\section{Bond evolution in the $(AsH_{2})_{20}$ ring molecule}

\begin{figure}[h]
  \centering
  \includegraphics[width = .9 \figurewidth]{AsH2_20atom_ring_BO_D.eps}
  \caption{\label{BOring} The values the bonding contribution, Wiberg
    bond number, and the center number for the four configurations in
    Fig. 18 of the main text. The lines are guides to the eye.}
\end{figure}

\section{AIM based analysis of bond evolution in symmetric $AsH_{2}-AsH-AsH_{2}$ trimer}

\begin{figure}[h]
  \centering
  \includegraphics[width = .9 \figurewidth]{As3H5_delocal_A.eps}
  \caption{\label{DI} Evolution of the the delocalization indices for electron densities associated with nearest-neighbor and multi-center bonds in the 4-electron/3-center arsenic trimer.}
\end{figure}

\bibliography{msSI}

%\end{document}

